Convergence of Goal-Oriented Adaptive Finite Element Methods for Semilinear Problems

In this article we develop a convergence theory for goal-oriented adaptive finite element algorithms designed for a class of second-order semilinear elliptic equations. We briefly discuss the target problem class, and introduce several related approximate dual problems that are crucial to both the analysis as well as to the development of a practical numerical method. We then review some standard facts concerning conforming finite element discretization and error-estimate-driven adaptive finite element methods (AFEM). We include a brief summary of a priori estimates for this class of semilinear problems, and then describe some goal-oriented variations of the standard approach to AFEM (GOAFEM). Following the recent approach of Mommer-Stevenson and Holst-Pollock for increasingly general linear problems, we first establish a quasi-error contraction result for the primal problem. We then develop some additional estimates that make it possible to establish contraction of the combined primal-dual quasi-error, and subsequently show convergence with respect to the quantity of interest. Finally, a sequence of numerical experiments are then carefully examined. It is observed that the behavior of the implementation follows the predictions of the theory.

==> environ.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% BEGIN: TeX/LaTeX/PDFLaTeX <Environment/Style> for Holst Group Papers
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\pdfoutput=1

%%% packages %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Graphics packages
\usepackage{color} % black,white,red,green,blue,cyan,magenta,yellow
\usepackage{ifpdf}
\ifpdf
    % PDF Graphics packages
    \usepackage[pdftex]{graphicx}
    %\usepackage{pdftricks}
    %\begin{psinputs}
    %  \usepackage{pstricks}
    %\end{psinputs}
    \usepackage[pdftex]{hyperref}
    %\usepackage{hyperref}
    \hypersetup{
        %bookmarks=true,        % show bookmarks bar?
        unicode=false,          % non-Latin characters in Acrobat’s bookmarks
        pdftoolbar=true,        % show Acrobat’s toolbar?
        pdfmenubar=true,        % show Acrobat’s menu?
        pdffitwindow=false,     % window fit to page when opened
        pdfstartview={FitH},    % fits the width of the page to the window
        pdftitle={MCP Article},      % title
        pdfauthor={Michael Holst},   % author
        pdfsubject={Mathematics},    % subject of the document
        pdfcreator={Michael Holst},  % creator of the document
        pdfproducer={Michael Holst}, % producer of the document
        pdfkeywords={PDE, analysis, mathematical physics}, % list of keywords
        pdfnewwindow=true,      % links in new window
        colorlinks=true,        % false: boxed links; true: colored links
        linkcolor=red,          % color of internal links
        citecolor=blue,         % color of links to bibliography
        filecolor=magenta,      % color of file links
        urlcolor=cyan           % color of external links
    }
    \def\myfigpng#1#2{\includegraphics[height=#2]{#1.png}}
    \def\myfigpdf#1#2{\includegraphics[height=#2]{#1.pdf}}
    \def\myfigps#1#2{\includegraphics[height=#2]{#1.pdf}}
    \def\myfig#1#2{\includegraphics[height=#2]{#1.png}}
    \typeout{====== Invoked by pdflatex ======================}
\else
    % DVI Graphics packages
    \usepackage{graphicx}
    \usepackage{pstricks}
    \newenvironment{pdfpic}{}{}
    \newcommand{\href}[2]{#2}
    \def\myfigpng#1#2{\includegraphics[height=#2]{#1}} % auto-select .ps/.eps
    \def\myfigpdf#1#2{\includegraphics[height=#2]{#1}} % auto-select .ps/.eps
    \def\myfigps#1#2{\includegraphics[height=#2]{#1}}  % auto-select .ps/.eps
    \def\myfig#1#2{\includegraphics[height=#2]{#1}}    % auto-select .ps/.eps
    \typeout{====== Invoked by latex ======================}
\fi

% Font packages
\usepackage{times}
\usepackage{amsfonts}

% Math packages
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{amsbsy}
\usepackage{amscd}

% Text packages
%\usepackage{multirow}
%\usepackage{array}
%\usepackage{bm}
\usepackage{enumerate}
%\usepackage{afterpage}
\usepackage{verbatim}
\usepackage{subfigure}
%\usepackage[algo2e,linesnumbered,ruled]{algorithm2e}

% SVMONO (Springer Book) specific packages
%\usepackage{mathptmx}
%\usepackage{helvet}
%\usepackage{courier}
%\usepackage{type1cm}         
%\usepackage{makeidx}        % allows index generation
%\usepackage{multicol}        % used for the two-column index
%\usepackage[bottom]{footmisc}% places footnotes at page bottom

% Long Chen's fancy chapter headings
%\usepackage[Lenny]{fncychap}
%\ChTitleVar{\LARGE \sffamily\bfseries}
%\usepackage{setspace}
%\setstretch{1.5}

%%%% theorems %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%%\newtheorem{theorem}{Theorem}[chapter]
%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{claim}[theorem]{Claim}
%\newtheorem{axiom}[theorem]{Axiom}
%\newtheorem{conjecture}[theorem]{Conjecture}
%\newtheorem{fact}[theorem]{Fact}
%\newtheorem{hypothesis}[theorem]{Hypothesis}
%\newtheorem{assumption}[theorem]{Assumption}
%\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{criterion}[theorem]{Criterion}
%\newtheorem{definition}[theorem]{Definition}
%\newtheorem{example}[theorem]{Example}
%\newtheorem{remark}[theorem]{Remark}
%\newtheorem{problem}[theorem]{Problem}
%\newtheorem{principle}[theorem]{Principle}
%\newtheorem{algorithm}[theorem]{Algorithm}
%
%% AMS-math specific things (comment out if not using package <amsmath.sty>)
%%\theoremstyle{definition}
%%\theoremstyle{remark}
%\numberwithin{equation}{section}  %amsmath command: tie counter to section
%
% Non-AMS-math specific things
%\numberwithin{section}{chapter}
%\numberwithin{equation}{chapter}
%\renewcommand{\theequation}{\arabic{section}.\arabic{equation}}

%%% label/itemize/enumerate styles %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\renewcommand{\theenumi}{\roman{enumi}}  % "iv"  labels for enumerate. 
%\renewcommand{\theenumi}{\arabic{enumi}} % "4"   labels for enumerate.
%\renewcommand{\labelenumi}{(\theenumi)}  % "(X)" labels in enumerate.
%\renewcommand{\labelenumi}{\theenumi.}   % "X."  labels in enumerate.
%\renewcommand{\thepage}{\arabic{page} - {\small DRAFT-1 \today}}

%%% environments %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% BEGIN: disable/enable margin notes
%-->disable margin notes
% \newcommand{\mnote}[1]{}
%-->enable margin notes
  \newcounter{mnote}
  \setcounter{mnote}{0}
  \newcommand{\mnote}[1]{\addtocounter{mnote}{1}
    \ensuremath{{}^{\bullet\arabic{mnote}}}
    \marginpar{\footnotesize\em\color{red}\ensuremath{\bullet\arabic{mnote}}#1}}
  \let\oldmarginpar\marginpar
    \renewcommand\marginpar[1]{\-\oldmarginpar[\raggedleft\footnotesize #1]%
    {\raggedright\footnotesize #1}}
% END: disable/enable margin notes

% lists
\newenvironment{enumerateY}
{\begin{list}{{\it(\roman{enumi})}}{
\usecounter{enumi}
\leftmargin 2.5em\topsep 0.5em\itemsep -0.0em\labelwidth 50.0em}}
{\end{list}}

\newenvironment{enumerateX}
{\begin{list}{\arabic{enumi})}{
\usecounter{enumi}
\leftmargin 2.5em\topsep 0.5em\itemsep -0.0em\labelwidth 50.0em}}
{\end{list}}

\newenvironment{itemizeX}
{\begin{list}{\labelitemi}{
\leftmargin 2.5em\topsep 0.5em\itemsep -0.0em\labelwidth 50.0em}}
{\end{list}}

\newenvironment{theoremX}
{\begin{trivlist}\em\item[\hskip\labelsep{\bf Theorem:}]}{\end{trivlist}}
\newenvironment{lemmaX}
{\begin{trivlist}\em\item[\hskip\labelsep{\bf Lemma:}]}{\end{trivlist}}
\newenvironment{corollaryX}
{\begin{trivlist}\em\item[\hskip\labelsep{\bf Corollary:}]}{\end{trivlist}}
\newenvironment{propositionX}
{\begin{trivlist}\em\item[\hskip\labelsep{\bf Proposition:}]}{\end{trivlist}}
\newenvironment{assumptionX}
{\begin{trivlist}\em\item[\hskip\labelsep{\bf Assumption:}]}{\end{trivlist}}
\newenvironment{algorithmX}
{\begin{trivlist}\em\item[\hskip\labelsep{\bf Algorithm:}]}{\end{trivlist}}
\newenvironment{definitionX}
{\begin{trivlist}\em\item[\hskip\labelsep{\bf Definition:}]}{\end{trivlist}}

\newenvironment{proofX}
{\begin{trivlist}\em\item[\hskip\labelsep{\bf Proof:}]}
{\vbox{\hrule\hbox{\vrule height1.4ex\hskip1.4ex\vrule}\hrule}\end{trivlist}}
\newenvironment{proofXO}
{\begin{trivlist}\em\item[\hskip\labelsep{\bf Proof Outline:}]}
{\vbox{\hrule\hbox{\vrule height1.4ex\hskip1.4ex\vrule}\hrule}\end{trivlist}}
\def\bproofX{{\bf Proof:}}
\def\eproofX{{\vbox{\hrule\hbox{\vrule height1.4ex\hskip1.4ex\vrule}\hrule}}}

%%% colors %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\definecolor{myblue}{rgb}{0.375,0.375,0.75}
\definecolor{myblue}{rgb}{0.2,0.2,0.7}
\definecolor{mygreen}{rgb}{0,0.6,0}
\definecolor{mycyan}{rgb}{0,0.6,0.6}
\definecolor{myred}{rgb}{0.9,0.2,0.2}
\definecolor{mymagenta}{rgb}{0.9,0.2,0.9}
\definecolor{mywhite}{rgb}{1.0,1.0,1.0}
\definecolor{myblack}{rgb}{0.0,0.0,0.0}

\def\Blue#1{{\color{myblue}#1}}
\def\Red#1{{\color{myred}#1}}
\def\Green#1{{\color{mygreen}#1}}
\def\Cyan#1{{\color{mycyan}#1}}
\def\Magenta#1{{\color{mymagenta}#1}}
\def\White#1{{\color{mywhite}#1}}
\def\Black#1{{\color{myblack}#1}}

%%% useful macros %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\linespacingX#1{{\renewcommand{\baselinestretch}{#1}\small\normalsize}}
\newcommand{\lined}{\hfill \hrule\hfill\vspace{1mm} \\}

%%% beamer support %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\usetheme[]{MJH}

%%% svmono override %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\newcommand{\preface}{}
%\newcommand{\motto}{}
%\newcommand{\subtitle}{}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% END: TeX/LaTeX/PDFLaTeX <Environment/Style> for Holst Group Papers
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


